Toward Designing Social Human-Robot Interactions for Deep Space Exploration

In planning for future human space exploration, it is important to consider how to design for uplifting interpersonal communications and social dynamics among crew members. What if embodied social robots could help to improve the overall team interaction experience in space? On Earth, social robots have been shown effective in providing companionship, relieving stress and anxiety, fostering connection among people, enhancing team performance, and mediating conflicts in human groups. In this paper, we introduce a set of novel research questions exploring social human-robot interactions in long-duration space exploration missions.

==> extra-materials.tex <==
\begin{comment}
Today, the crafts used in these early space exploration programs would be classified as isolated and confined environments (ICE): in-habitants are physically separated from other people and conventional support systems, and they are confined to a small capsule~\cite{Palinkas2001-PsychosocialIL,Suedfeld2000-EnvironmentalPC}. Submariners, inhabitants of Antarctic bases. 

Looking out the ISS windows at earth has been cited as a highly rewarding, psychologically enriching, and even atranscendent activity, with crew members tending to voluntarily take hundreds of pictures of earth [17].
\end{comment}

\begin{comment}
 ~\cite{SALAMON2018-ApplicationVR}
Human exploration of the solar system brings a host of environmental and engineering challenges. Among the most important factors in crew health and human performance is the preservation of mental health. The mental well-being of astronaut crews is a significant issue affecting the success of long-duration space missions,such as habitation on or around the Moon, Mars exploration, and eventual colonization of the solar system. If mental health is not properly addressed,these missions will be at risk. Upkeep of mental health will be especially difficult on long duration missions because many of the support systems available to crews on shorter missions will not be available. 
\end{comment}

\begin{comment}
 (b) mental disorders could develop should adverse behavioral conditions be undetected and unmitigated’’ (NASA, 2019)~\cite{nasa_2020}. 
(NASA, 2019).
\end{comment}

\begin{comment}
~\cite{Huntsberger2010-EnvisioningCR}
Fielding robots in space places some restraints on what can be done due to limited computing capabilities, mass and
volume constraints, low bandwidth communication channels coupled with oftentimes long delays, and power issues.
CARACaS has been tested extensively on Unmanned Surface Vehicles (USV’s) under US Navy contracts as well
\end{comment}

\begin{comment}


 "While in zero gravity, the embodied social agent interacted with people on cognitive, creative, and social tasks with varying degrees of proactive behavior. We collected physiological, audio, and video data of the experience as individuals completed a series of tasks with the agent with the goal of designing agents that can enable us to be more socially connected."
 
 https://www.nikhitasingh.com/work/zero-g-robtos 
\end{comment}

\begin{comment}

To assess a a participant’s perception of a robot's social attributes, the Robotic Social Attributes Scale (RoSAS)~\cite{Carpinella2017-RoboticSA} is often used. 

\end{comment}

\begin{comment}
 Numerous HRI studies demonstrated that people respond to robots in unique ways~\cite{Deng2019-EmbodimentSI} compared to other non-physically embodied agents
 
 In MHRI, an agent's physical embodiment has also been shown to improve human group’s social perception of the agent~\cite{Shamekhi2018-FaceVE}. 
\end{comment}


Another challenge is the communication between people in space and on Earth. As astronaut Scott Kelly describes in the Time documentary A Year in Space~\cite{Kelly-YearS}, the experience can be incredibly isolating despite several forms of digital and voice communication, including phone calls, video conferencing, and email. Shortcomings of these modes of communication lie in their inability to translate emotion effectively, failure to facilitate shared experiences, lack of physical feedback, and the resulting perceived lack of control. The psychological effects of these limitations can become heightened over time, and peak during moments when the family on Earth is in need of support. In addition, the lack of enriching connectivity between space and earth also leads to numerous absences from the astronaut's family in particular, hindering the parental involvement of astronauts such as their absence of important milestones, events, and celebrations in the lives of their children. Prior work showed that retired astronauts wished they had been “much more involved” than they had been were in intellectual, emotional, spiritual, and physical development of their children (e.g., sharing activities/interests, and companionship)~\cite{JOHNSON2018-BeingFD}. Overall, it is important to consider how we design for social connectivity between people on Earth and in space.

During nine-month one-way voyage to Mars, earth will shrink into the background of space as a point of light (dubbed the“Earth out of view phenomenon”~\cite{Kanas2008-SpacePP}), and the communication lag due to distance between the craft and Earth will become as long as twenty minutes on average[20]. 

Daily life will take place in small and confined areas, for durations extending into years. The dangers of the extreme environment of space are ever-present, and failure of critical equipment or components can lead to death.

% Salamon et al~\cite{SALAMON2018-ApplicationVR} examine the use of immersive virtual reality (VR) simulations to maintain healthy mental states in astronaut crews who are removed from the essential comforts typically associated with terrestrial life.

%immersive virtual reality (VR) applications to maintain healthy mental states in astronaut crews~\cite{SALAMON2018-ApplicationVR}. 

From C3PO in Star Wars to Rosie the Maid in The Jetsons, the idea of robots in space has been well explored in fiction universe. 


% In this paper, we first provide an overview of social HRI on Earth with regards to (1) how social robots can positively impact human group dynamics and processes, (2) how social robots can promote well-being and performance of individuals in various ways, and (3) . Based on this exploration, we present the opportunities for researchers and designers in the context of social human-robot interaction design in deep space mission. In particular, we highlight three future directions of SpaceHRI research, namely mental wellbeing of astronauts, connectivity of people between Earth and space, and social-emotional dynamics and processes of the space team. 



%% project: Astronaut Affect Recognition Using Speech Technology using the Apollo 11 Fearless Steps Corpus
%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
~\cite{Landon2018TeamworkAC}
TEAMWORK
The scientific study of teamwork in the context of spaceflight has uncovered a considerable
amount of knowledge over the past 20 years. Although much is known about the underlying
factors and processes of teamwork, much is left to be discovered for teams who will be operating
in extreme isolation and confinement during a future Mars mission. Special considerations must
be made to enhance teamwork and team well-being for multi-year missions during which the
small team will live and work together.

Performance support tools, such as guided team debriefs, were designed to address both the task performance and the dynamics of teams living together,

teamwork skills are critical. One astronaut stated, “Task disruptions may happen more often; but interpersonal [disruptions are] more problematic and they need more discussion to overcome” (Maynard & Kennedy, 2016, p. 33).

Successfully negotiating conflict, planning together as a team, making decisions as a
team, and practicing shared leadership should receive extensive attention long before a team launches on a space
mission.
\end{comment}



\begin{comment}
~\cite{Rosenfeld2019-HumanAI}
we suggest that advances in human-agent interaction technologies can assist astronauts in their missions by automatically reliving some of the challenges astronauts face. However, it is also our claim that these possible contributions are bounded by the agents’ ability to proficiently model, adapt and personalize their behavior to each astronaut and/or to a group of astronauts, with minimal to no human intervention.

The analogue astronauts further pointed out two possible avenues for such contributions:
(1) Assisting each astronaut individually.
(2) Assisting astronauts as a group.
\end{comment}

%%%%% PAPERS %%%%%%%% 
% Gardening for Therapeutic People-Plant Interactions during Long-Duration Space Missions
% https://www.degruyter.com/document/doi/10.1515/opag-2017-0001/html

% The nature of conflict for teams in isolated, confined, and extreme environments
% https://www.sciencedirect.com/science/article/abs/pii/S0094576521000047

% Astrobee Robot Software: Enabling Mobile Autonomy on the ISS
% http://brian.coltin.org/pub/fluckiger2018astrobee.pdf


